Experimental Realization and Characterization of Stabilized Pair Coherent States

The pair coherent state (PCS) is a theoretical extension of the Glauber coherent state to two harmonic oscillators. It is an interesting class of non-Gaussian continuous-variable entangled state and is also at the heart of a promising quantum error correction code: the pair cat code. Here we report an experimental demonstration of the pair coherent state of microwave photons in two superconducting cavities. We implement a cross-cavity pair-photon driven dissipation process, which conserves the photon number difference between cavities and stabilizes the state to a specific complex amplitude. We further introduce a technique of quantum subspace tomography, which enables direct measurements of individual coherence elements of a high-dimensional quantum state without global tomographic reconstruction. We characterize our two-mode quantum state with up to 4 photons in each cavity using this subspace tomography together with direct measurements of the photon number difference and the joint Wigner function. We identify the spurious cross-Kerr interaction between the cavities and our dissipative reservoir mode as a prominent dephasing channel that limits the steady-state coherence in our current scheme. Our experiment provides a set of reservoir engineering and state characterization tools to study quantum optics and implement multi-mode bosonic codes in superconducting circuits.

==> backup.tex <==
\begin{document}



The working principle is to entangle a small subspace $\mathcal{S}$ of a larger quantum system with the $\ket{e}$ state of a three-level ancilla, allowing for tomographic measurements within $\mathcal{S}$ in an isolated manner by mapping observables with the $\ket{e}\rightarrow\ket{f}$ transition.

The system-ancilla state following the first-step entanglement is:
\begin{align}
    \rho_\textrm{tot}=\rho_\mathcal{SS}\Pi_{ee}+\rho_\mathcal{EE}\Pi_{gg}+\rho_\mathcal{SE}\Pi_{eg}+\rho_\mathcal{ES}\Pi_{ge}
    \label{eq:tomostate}
\end{align}
where $\Pi_{ij}$ are the ancilla state projectors $\ket{i}\bra{j}$, and %$\rho_\mathcal{SS}, \rho_\mathcal{EE}, \rho_\mathcal{SE}, \rho_\mathcal{ES}$ 
$\rho_{ij}$ are the four density matrix blocks of the system, with $\mathcal{E}$ representing the rest of the system Hilbert space orthogonal to $\mathcal{S}$.  We note that, in principle, a projective measurement of the ancilla followed by a post selection can be used to immediately project the state to $\rho_\mathcal{SS}$.  However, this would require highly ideal measurement capabilities with high fidelity, quantum non-demolition on the ancilla, and no cross-talk back-action on the system.  Instead, we can apply a convenient unitary operation $\hat{U}$, such as a displacement, to transform the cavity state, followed by mapping a set of POVM of the system, $\{M_0, M_1\}$, to the $\ket{e}-\ket{f}$ transition, giving:
\begin{align}
    \hat{U}_\mathrm{tot} &= [(\Pi_{ee}+\Pi_{ff})\hat{M}_0+(\Pi_{fe}+\Pi_{ef})\hat{M}_1]\hat{U}\\
    \hat{U} &= \Pi_{ee} \hat{U}_e + \Pi_{gg} \hat{U}_g + \Pi_{ff} \hat{U}_f
\end{align}
where $\hat{U}_i$ is the cavity unitary when the ancilla is in $\ket{i}$.  Finally we read out the ancilla (to distinguish $\ket{f}$ vs.~$\ket{e}$), effectively measuring $\textrm{Tr}[\hat{M}_1\hat{U}_e\rho_\mathcal{SS}\hat{U}^\dagger_e\hat{M}^\dagger_1]$. Crucially, one can tailor the measurement operator $\hat{M}_1\hat{U}_e$ completely disregarding $\hat{U}_g$ or other spurious transformation occurring outside the subspace $\mathcal{S}$ because they do not contribute to the readout contrast.  


\subsection*{prediction of distribution of delta states from loss}
TODO: SEAN

\begin{figure*}[tbp]
    \centering
    \includegraphics[scale=1]{delta_dist_v2.pdf}
    \caption{\textbf{$\delta$ state hopping from single photon loss.} a Plot of the $C_{\delta}$ coefficients from eq. TODO for different $delta$ values assuming a pair coherent state amplitude of $\gamma = 1.25$ and loss rates of $(200\mu s)^{-1}$ and $(216\mu s)^{-1}$ for cavity a and b respectively. b) Diagrammatic representation of single photon loss causing hopping to different $\delta$ states where the right (left) pointing red arrows represent a photon loss event from cavity b (a) with the respective rates as indicated on the figure.
}
\end{figure*}

\begin{figure*}[tbp]
    \centering
    \includegraphics[scale=.45]{dm_reconstruction.pdf}
    \caption{\textbf{Density matrix reconstruction} a) Comparison of the $Re(\alpha)$ vs. $Re(\beta)$ 2-D Wigner cut from experiment (left) against the reconstructed density matrix (right). b) Color plot of the reconstructed density matrix with only the elements corresponding to the $delta = -1,0,1$ states.
}
\end{figure*}

\begin{figure*}[tbp]
    \centering
    \includegraphics[scale=.38]{dm_reconstruction_v3.pdf}
    \caption{\textbf{Density matrix reconstruction} a-d) Comparison of the 2-D Wigner cuts from experiment (left) against the reconstructed density matrix (right) for $Re(\alpha) vs. Re(\beta)$, $Re(\alpha) vs. Im(\alpha)$, $Re(\alpha) vs. Im(\beta)$, $Im(\alpha) vs. Im(\beta)$ respectively. b) Color plot of the reconstructed density matrix with only the elements corresponding to the $delta = -1,0,1$ states.
}
\end{figure*}



Given a pair coherent state that is allowed to freely evolve with single photon loss from each cavity while being stabilized by two photon loss, we would like to be able to predict the distribution of the populations of each $\delta$ state by finding the $C_{\delta}$ coefficients in the following equation:
\begin{equation}
    \rho(t=\infty) = \sum_{\delta=-\infty}^\infty C_\delta \ket{\gamma, \delta}\bra{\gamma, \delta}
\end{equation}
We will be working in the regime where the two photon loss stabilization is much stronger than the single photon loss ($\kappa_{ab}>>\kappa_{a},\kappa_{b}$) so we can assume that after a single photon loss event happens, creating a change in $\delta$ by 1, the state can be treated as though it is effectively instantaneously stabilized to a pair coherent state of the new $\delta$ while maintaining the state amplitude $\gamma$. 
With this assumption in place, we can treat the problem as a simple equilibrium solution to the different delta states and their respective probabilities to jump to neighboring states based off the photon populations in each cavity, as illustrated in Fig.~E1(b). We can represent the photon populations at a given $\gamma$ and $\delta$ ($\Bar{n}_{a}(\gamma ,\delta)$) in cavity $a$ with the following expression ~\cite{agarwal_generation_1986}:
\begin{align}
    \Bar{n}_{a}(\gamma ,\delta)=\frac{N_{\gamma,\delta}^{2}}{N_{\gamma,\delta+1}^{2}}|\gamma|^{2}+\delta ,\\\nonumber   N_{\gamma,\delta} = ((i|\gamma|)^{-\delta}J_{\delta}(2i|\gamma|))^{-1/2}
\end{align}
Where $J_{\delta}$ is the bessel function of the first kind of order $\delta$. One can then get the photon number in $b$ ($\Bar{n}_{b}(\gamma ,\delta)$) by subtracting the $\delta$ from Eq.~(16). We can now construct the rates of photon loss from cavity $a/b$ with a $\gamma$ and $\delta$ being $\kappa_{i}\Bar{n}_{a/b}(\gamma,\delta)$. Treating each state then with an outgoing rate due to photon loss and an incoming rate from photon loss of neighboring states allows us to create the following equilibrium equation for each $\delta$ value:
\begin{align}
    C_{\delta}(\kappa_{a}\Bar{n}_{a}(\gamma ,\delta)+\kappa_{b}\Bar{n}_{b}(\gamma ,\delta))-C_{\delta+1}(\kappa_{a}\Bar{n}_{a}(\gamma ,\delta)) \\\nonumber - C_{\delta-1}(\kappa_{b}\Bar{n}_{b}(\gamma ,\delta)) = 0
\end{align}
Numerically solving this set of coupled equations for all the desired $\delta$ states yields a solution for the distribution of $C_{\delta}$ values with an example distribution plotted out in Fig.~E1(b).




\begin{figure*}[tbp]
    \centering
%    \includegraphics[scale=1]{fig3_1-27.pdf}
    \caption{\textbf{Time domain measurement of the pair coherent state at longer times. a} Showing the population of each state $\delta=0$ state with time and decaying over long times, the best pair coherent state is observed at $\Delta t=????$,    \textbf{b} We also measure the population of $\delta=+1,-1$ which is the sum of population of all the states with one more photon in cavity A and cavity B respectively. \textbf{c}Similarly we also measure the $\delta=0, 2$ states over long timescale to find that the population becomes equal after $150\mu s$ suggesting that we do not have a pair coherent state that can live for longer timescales like these.  
}
\end{figure*}


\subsection*{math dump}


\begin{equation*}
    \xi\approx\sqrt{\Delta_\text{Stark}/2 \alpha_q}
\end{equation*}

\begin{equation}
     g_{ab} = \sqrt{\frac{\chi_{qa} \chi_{qb} \chi_{rq}\Delta_\text{Stark}}{\chi_{qq}^2}} 
\end{equation}

\begin{equation}
     k_{ab} = 4\frac{\chi_{qa} \chi_{qb} \chi_{rq}}{\chi_{qq}^2 \kappa_r}\Delta_\text{Stark}
\end{equation}

\begin{equation}
     k_{ab} = 4\frac{\chi_{qa} \chi_{qb} \chi_{rq}}{\chi_{qq}^2 \kappa_r}\Delta_\text{Stark}
\end{equation}

From fit: $\epsilon_{ab} \approx (15.9 kHz) * 2 \pi$, $\kappa_{ab} \approx (12.7 kHz) * 2\pi$ which gives
$|\gamma| = 2 \frac{\epsilon_{ab}}{\kappa_{ab}} = 2.5$

$\epsilon_{ab} = -2ig_{ab} \epsilon_d/\kappa_r$ and pair photon dissipation $\kappa_{ab} = 4 |g_{ab}|^2/\kappa_r$

\begin{equation}
    g_{ab} = \sqrt{\kappa_r \kappa_{ab}}/2
\end{equation}

\begin{equation}
    |\epsilon_d| = \frac{\epsilon_{ab}\kappa_r}{2\g_ab}=  \epsilon_{ab}\sqrt{\kappa_r/\kappa_{ab}}
\end{equation}


\begin{equation}
    \Dot{\rho} = -i(\hat{H}_{eff}\rho - \rho \hat{H}_{eff}^\dagger) + \sum_j \kappa_j \hat{L}_j \rho \hat{L}_j^\dagger
\end{equation}

\begin{equation}
    \hat{H}_{eff} = \hat{H} - i \sum_J \frac{\kappa_j}{2}\hat{L}_j^\dagger \hat{L}_j
\end{equation}

\begin{equation}
    \hat{H}_{eff} = \epsilon_{ab} \hat{a}\hat{b} + \epsilon_{ab}^* \hat{a}^\dagger\hat{b}^\dagger + K_{eff}\hat{a}^\dagger\hat{b}^\dagger \hat{a}\hat{b} - i \frac{\kappa_{ab}}{2}\hat{a}^\dagger\hat{b}^\dagger \hat{a}\hat{b}
\end{equation}


\begin{align}
    \Dot{\rho} &= (\epsilon_{ab} \gamma - \epsilon_{ab}^* \gamma^* + i \kappa_{ab} |\gamma|^2)\rho \\\nonumber &+ (\epsilon^* + K_{eff}\gamma - i\frac{\kappa_{ab}}{2} \gamma)\hat{a}^\dagger\hat{b}^\dagger \rho \\\nonumber &- (\epsilon + K_{eff}\gamma^* + i\frac{\kappa_{ab}}{2} \gamma^*) \rho \hat{a}\hat{b}
\end{align}

\begin{equation}
    \gamma = \frac{\epsilon^*}{\frac{i\kappa}{2}-K_{eff}}
\end{equation}


\begin{equation}
    \rho(t=\infty) = \sum_{\delta=-\infty}^\infty C_\delta \ket{\gamma, \delta}\bra{\gamma, \delta}
\end{equation}


\begin{equation}
    \hat{P}_J = \hat{P}_a\hat{P}_b = e^{i\pi \hat{a}^\dagger \hat{a}} e^{i\pi \hat{b}^\dagger \hat{b}}
\end{equation}


\subsection{Density Matrix Reconstruction}
TODO: SEAN

To reconstruct the density matrix from a set of wigner tomography slices with varying displacements on both cavities, we implemented a general N-mode numerical density matrix reconstruction method outlined in~\cite{reinhold_controlling_2019}. We can treat the wigner tomography data as general measurements $M$ where we can express the measurement outcomes $x$ in terms of the density matrix $\rho$ as:
\begin{equation}
    x = Tr{(M\rho)}=\sum_{ij} M_{ij}\rho_{ji}\equiv \langle\braket{M}{\rho}\rangle
\end{equation}
Then taking $N_{exp}$ measurements gives us the following relation:
\begin{equation}
    \vec{x} = (\sum_{i}^{N_{exp}}\ket{x_{i}}\langle\bra{M_{i}})\ket{\rho}\rangle \equiv \mathscr{M}\ket{\rho}\rangle
\end{equation}
Since $\mathscr{M}$ will not generally be a square matrix, we can take a pseudo inverse to get the closest approximate solution using the Moore-Penrose pseudo-inverse:
\begin{equation}
    minimize|\mathscr{M}\ket{\rho}\rangle - \vec{x}| \rightarrow \ket{\rho_{least-sq}}\rangle = (\mathscr{M}\mathscr{M}^{T})^{-1}M^{T}\vec{x}
\end{equation}
To try to constrain the physicality of the reconstruction, we added a lagrange multiplier constraint to the reconstruction that fixes the density matrix on diagonal population values to what was observed in the transmon spectroscopy data plotted in Fig.~2(b):

\begin{equation}
\begin{pmatrix}
\mathscr{M}^{T}\mathscr{M} & C^{T}\\
C & 0
\end{pmatrix}
\begin{pmatrix}
\vec{\rho}\\
\vec{\lambda}
\end{pmatrix}
= 
\begin{pmatrix}
\mathscr{M}^{T}\vec{x}\\
\vec{d}
\end{pmatrix}
\end{equation}

Where $C\vec{\rho} = \vec{d}$ represents the constraints. Since the input diagonals are all real and with the trace equaling one, further physicality constraints on the matrix, such as positive definite eigenvalues and $Tr(\rho)=1$, are unnecessary.

The density matrix yielded from this procedure is plotted in a reduced form showing only the $\delta = -1,0,1$ components in Fig.~E2(b), with a side by side wigner cut comparison against the experimental values displayed in Fig.~E2(a).\\


\section{Additional data}

\subsection{Superposition of different delta}
\begin{figure}[tbp]
    \centering
    \includegraphics[scale=.95]{fig9_09122022_2.pdf}
    \caption{Comparing the Wigner function of a superposition of two PCS in the experiment and the simulation. 
    (a) %Measured 2D slice of a joint Wigner function for the $(\ket{\gamma, 0}+\ket{\gamma,1})/\sqrt2$ superposition state at an angle that corresponds to a Re[$\alpha$]-Re[$\beta$] cut for the $\ket{\gamma, \delta=1}$ state as shown in the Fig.~\ref{fig:PC_4}(f).
    Measured Re[$\alpha$]-Re[$\beta$] cut of the joint Wigner function $W(\alpha,\beta)$ for an experimental two-cavity state of the expected form $(\ket{\gamma e^{i\phi}, 0}+e^{i\varphi}\ket{\gamma,1})/\sqrt2$.  The cavity rotating frame used for the tomography (phase definition of $\alpha, \beta$) is defined such that $\gamma$ is real. 
    %The $\ket{\gamma,\delta=0}$ state in the experiment has a phase 2 radians lower than the $\ket{\gamma,\delta=1}$ state. 
    The Wigner function is measured at $t_{w}=4.5$ $\mu$s after the $t=15$ $\mu$s of stabilizing pump on a $(\ket{00}+\ket{01})/\sqrt{2}$.  The cavity free evolution during $t_w$ causes non-zero $\phi$ and $\varphi$.  
    (b) Simulated Wigner function of the same two-PCS superposition state using the same $t_{w}=4.5$ $\mu$s and the same stabilizing pumping parameters.  The cavity frame for tomography is similarly defined for make $\gamma$ real in order to simulate the same condition as in the experiment.  The relative phases of the superposition are consistent with the experiment as demonstrated by the similar features in the Wigner function.  %between the $\ket{\gamma,\delta=0}$ and the $\ket{\gamma, \delta=1}$ states are comparable to the ones in the experiment since we can see that the Wigner shows similar features.      
}\label{fig:superposition}
\end{figure}

\end{document}

